A Contour Stochastic Gradient Langevin Dynamics Algorithm for Simulations of Multi-modal Distributions

We propose an adaptively weighted stochastic gradient Langevin dynamics algorithm (SGLD), so-called contour stochastic gradient Langevin dynamics (CSGLD), for Bayesian learning in big data statistics. The proposed algorithm is essentially a \emph{scalable dynamic importance sampler}, which automatically \emph{flattens} the target distribution such that the simulation for a multi-modal distribution can be greatly facilitated. Theoretically, we prove a stability condition and establish the asymptotic convergence of the self-adapting parameter to a {\it unique fixed-point}, regardless of the non-convexity of the original energy function; we also present an error analysis for the weighted averaging estimators. Empirically, the CSGLD algorithm is tested on multiple benchmark datasets including CIFAR10 and CIFAR100. The numerical results indicate its superiority to avoid the local trap problem in training deep neural networks.

==> NeurIPS 2020 Contour Langevin Dynamics - arXiv v2/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> NeurIPS 2020 Contour Langevin Dynamics - arXiv v2/supp_content.tex <==

% \setcounter{lemma}{0}
\renewcommand\thesection{\Alph{section}}
% \renewcommand\thesubsection{\arabic{subsection}}
% \renewcommand{\thelemma}{\Alph{section}\arabic{lemma}}
\def\qed{ \ \vrule width.2cm height.2cm depth0cm\smallskip}
\newcommand\myeq{\stackrel{\mathclap{\normalfont\mbox{A}}}{=}}

\newcommand{\la}{\langle}
\def \proof{{\noindent \bf Proof\quad}}

The supplementary material is organized as follows: Section \ref{review} provides a  review 
for the related methodologies, Section \ref{convergence} proves the stability condition and convergence of the self-adapting parameter, Section \ref{ergodicity} establishes the ergodicity of the contour stochastic gradient Langevin dynamics (CSGLD) algorithm,  and Section \ref{ext} provides more discussions for the algorithm. 

\section{Background on stochastic approximation and Poisson equation}
\label{review}

\subsection{Stochastic approximation}
Stochastic approximation \citep{Albert90} provides a standard framework for the development of adaptive algorithms. Given a random field function $\widetilde H(\bm{\btheta}, \bm{\bx})$, the goal of the stochastic approximation algorithm is to find the solution to the  mean-field equation $h(\btheta)=0$, i.e., solving
\begin{equation*}
\begin{split}
\label{sa00}
h(\btheta)&=\int_{\MX} \widetilde H(\bm{\theta}, \bm{\bx}) \varpi_{\bm{\theta}}(d\bm{\bx})=0,
\end{split}
\end{equation*}
where $\bx\in \MX \subset \mathbb{R}^d$, $\btheta\in\bTheta \subset \mathbb{R}^{m}$, $\widetilde H(\btheta,\bx)$ is a random field 
function and $\varpi_{\btheta}(\bx)$ is a distribution function of $\bx$ depending on the parameter $\btheta$. The stochastic approximation  algorithm works by repeating the following iterations
\begin{itemize}
\item[(1)] Draw $\bm{x}_{k+1}\sim\Pi_{\bm{\theta_{k}}}(\bm{x}_{k}, \cdot)$, where $\Pi_{\bm{\theta_{k}}}(\bm{x}_{k}, \cdot)$ is a transition kernel that admits $ \varpi_{\bm{\theta}_{k}}(\bm{x})$ as
the invariant distribution,

\item[(2)] Update $\bm{\theta}_{k+1}=\bm{\theta}_{k}+\omega_{k+1} \widetilde H(\bm{\theta}_{k}, \bm{x}_{k+1})+\omega_{k+1}^2 \rho(\bm{\theta}_{k}, \bm{x}_{k+1}),$
where $\rho(\cdot,\cdot)$ denotes a bias term. 
\end{itemize}

The algorithm differs from the Robbins–Monro algorithm \citep{RobbinsM1951} in that $\bx$ is simulated from a transition kernel $\Pi_{\bm{\theta_{k}}}(\cdot, \cdot)$ instead of the exact distribution $\varpi_{\bm{\theta}_{k}}(\cdot)$. As a result, a Markov state-dependent noise $\widetilde H(\btheta_k, \bx_{k+1})-h(\btheta_k)$ is generated, which requires some regularity conditions to control the fluctuation $\sum_k \Pi_{\btheta}^k (\widetilde H(\btheta, \bx)-h(\btheta))$. Moreover, it supports a more general form where a bounded bias term $\rho(\cdot,\cdot)$ is allowed without affecting the theoretical properties of the algorithm.

\subsection{Poisson equation}

Stochastic approximation generates a nonhomogeneous Markov chain $\{(\bx_k, \btheta_k)\}_{k=1}^{\infty}$, for which the convergence theory can be studied based on the Poisson equation 
\begin{equation*}
    \mu_{\btheta}(\bm{x})-\mathrm{\Pi}_{\bm{\theta}}\mu_{\bm{\theta}}(\bm{x})=\widetilde H(\bm{\theta}, \bm{x})-h(\bm{\theta}),
\end{equation*}
where $\Pi_{\bm{\theta}}(\bm{x}, A)$ is the transition kernel for any Borel subset $A\subset \MX$ and $\mu_{\btheta}(\cdot)$ is a function on $\MX$.
The solution to the Poisson equation exists when 
the following series converges:
\begin{equation*}
    \mu_{\btheta}(\bx):=\sum_{k\geq 0} \Pi_{\btheta}^k (\widetilde H(\btheta, \bx)-h(\btheta)).
\end{equation*}
That is, the consistency of the estimator $\btheta$ can be established by controlling the perturbations of $\sum_{k \geq 0} \Pi_{\btheta}^k (\widetilde H(\btheta, \bx)-h(\btheta))$ via imposing some regularity conditions on $\mu_{\btheta}(\cdot)$. Towards this goal, \citet{Albert90} gave 
the following regularity conditions on $\mu_{\btheta}(\cdot)$ to ensure the convergence of the adaptive algorithm:

{\it There exist a function  $V: \MX \to [1,\infty)$, and a constant $C$ such that for all $\bm{\theta}, \bm{\theta}'\in \bm{\bTheta}$,}
\begin{equation*}
\begin{split}
\|\mathrm{\Pi}_{\bm{\theta}}\mu_{\btheta}(\bx)\|&\leq C V(\bx),\quad
\|\mathrm{\Pi}_{\bm{\theta}}\mu_{\bm{\theta}}(\bx)-\mathrm{\Pi}_{\bm{\theta'}}\mu_{\bm{\theta'}}(\bx)\|\leq C\|\bm{\theta}-\bm{\theta}'\| V(\bx),  \quad 
\E[V(\bx)]\leq \infty,\\
\end{split}
\end{equation*}
which requires only the first order smoothness. In contrast, the ergodicity theory by \citet{mattingly10} and \citet{VollmerZW2016} 
relies on the much stronger 4th order smoothness.

% Poisson equation has been widely used in ergodic theory and adaptive algorithms to prove the desired limit of a time-average. Consider the infinitesimal generator $\mathcal{L}$ of the overdamped Langevin diffusion and let $\phi$ solve the Poisson equation
% \begin{equation}
%     \mathcal{L}\phi(\bx):=g-\bar g, 
% \end{equation}
% where $g$ is a test function and $\bar g$ is the expectation of $g$ over the Gibbs measure, defined as $\bar g=\int_{\bX}g(\bx) \varpi(d\bx)$. It is known that in a d-dimensional torus $\mathbb{T}^d$ and under elliptic settings, there is a unique solution for the Poisson equation, which is at least k+2-order smooth given a k-order smooth test function $g$ \citep{mattingly10}. To extend the ergodic average from $\mathbb{T}^d$ to $\mathbb{R}^d$, \citep{VollmerZW2016} established the required assumptions to establish the existence of smooth solutions of Poisson equation for stochastic gradient Langevin dynamics.


\section{Stability and convergence analysis for CSGLD} \label{convergence}

\subsection{CSGLD algorithm} \label{Alg:app}

To make the theory more general, we slightly extend CSGLD by allowing a higher order bias term. The resulting algorithm works by iterating between the following two steps:
\begin{itemize}
\item[(1)] Sample $\bm{x}_{k+1}=\bx_k- \epsilon_k\nabla_{\bx} \widetilde L(\bx_k, \btheta_k)+\mathcal{N}({0, 2\epsilon_k \tau\bm{I}}), \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (\text{S}_1)$

\item[(2)] Update $\bm{\theta}_{k+1}=\bm{\theta}_{k}+\omega_{k+1} \widetilde H(\bm{\theta}_{k}, \bm{x}_{k+1})
+\omega_{k+1}^2 \rho(\bm{\theta}_{k}, \bm{x}_{k+1}),
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  (\text{S}_2)$
\end{itemize}
where $\epsilon_k$ is the learning rate, $\omega_{k+1}$ is the step size, $\nabla_{\bx} \widetilde L(\bx, \btheta)$ is the 
stochastic gradient given by 
\begin{equation}
    \nabla_{\bx} \widetilde{L}(\bx,\btheta)= \frac{N}{n} \left[1+ 
   \frac{\zeta\tau}{\Delta u}  \left(\textcolor{black}{\log \theta(J_{\widetilde U}(\bx))-\log\theta((J_{\widetilde U}(\bx)-1)\vee 1)} \right) \right]  
    \nabla_{\bx} \widetilde U(\bx),
\end{equation}
$\widetilde H(\btheta,\bx)=(\widetilde H_1(\btheta,\bx), \ldots, 
 \widetilde H_m(\btheta,\bx))$ is a random field function with
\begin{equation}
\label{def_tilde_H}
     \widetilde H_i(\btheta,\bx)={\theta}^{\zeta}(J_{\widetilde U}(\bx))\left(1_{i= J_{\widetilde U}(\bx)}-{\theta}(i)\right), \quad i=1,2,\ldots,m,
\end{equation}
for some constant $\zeta>0$, and $\rho(\btheta_k,\bx_{k+1})$ is a bias term.

\subsection{Convergence of parameter estimation} 
\label{App:convergence}

To establish the convergence of $\btheta_k$, we make the following assumptions:


\begin{assump}[Compactness] \label{ass2a} 
The space $\Theta$ is compact such that $\inf_{\Theta} \theta(i) >0$ for any  $i\in \{1,2,\ldots,m\}$; the perturbation term $\rho(\btheta, \bx)$ is also uniformly bounded for any $\bx \in \MX$ and $\btheta \in \bTheta$.
\end{assump}

To simplify the proof, we consider a slightly stronger assumption such that $\inf_{\Theta} \theta(i)>0$ holds for any $i \in \{1,2,\ldots,m\}$. To relax this assumption, we refer interested readers to \citet{Fort15} where the recurrence property was proved for the sequence $\{\btheta_k\}_{k\geq 1}$ of a similar algorithm. Such a property guarantees $\btheta_k$ to visit often 
enough to a desired compact space, rendering the convergence of the sequence. 

By Assumption \ref{ass2a} and Eq.(\ref{def_tilde_H}), it is easy to conclude that there exists a constant $Q>0$ such that for any $\btheta\in \bTheta$ and $\bx \in \MX$, 
\begin{equation}
\label{compactness}
     \|\btheta\|\leq Q, \quad  
     \|\widetilde H(\btheta, \bx)\|\leq Q, \quad 
     \|\rho(\btheta, \bx)\|\leq Q.
\end{equation}


 
% \begin{assump}[Smoothness]
% \label{ass2}
% $\nabla_{\bx} L(\bm{\xeta}, \bm{\theta})$ is $M$-smooth, namely, for any $\bx, \bx'\in \bX$, $\bm{\theta}, \bm{\theta}'\in \bTheta$,
% \begin{equation}
% \label{ass_2_1_eq}
% \begin{split}
% \|\nabla_{\bx} L(\bx, \btheta)-\nabla_{\bx} L(\bm{\bx}', \btheta')\| & \leq M\|\bx-\bx'\|+M\|\btheta-\btheta'\|, \\
% %\|\nabla_{\bx} L(\bx, \btheta)-\nabla_{\bx} L(\bm{\bx}, \btheta')\| & \leq M\|\btheta-\btheta'\|, \\
% \end{split}
% \end{equation}
% \end{assump}

\textcolor{black}{\begin{assump}[Smoothness]
\label{ass2}
$U(\bm{\xeta})$ is $M$-smooth; that is, there exists a constant $M>0$ such that for any $\bx, \bx'\in \MX$,
\begin{equation}
\label{ass_2_1_eq}
\begin{split}
\|\nabla_{\bx} U(\bx)-\nabla_{\bx} U(\bm{\bx}')\| & \leq M\|\bx-\bx'\|. \\
\end{split}
\end{equation}
\end{assump}}

Smoothness is a standard assumption in the study of convergence of SGLD, see e.g. \citet{Maxim17,Xu18}. 
 
 

\begin{assump}[Dissipativity]
\label{ass3}
 There exist constants $\tilde{m}>0$ and $\tilde{b}\geq 0$ such that for any $\bx \in \MX$ and $\btheta \in \bTheta$, 
\label{ass_dissipative}
\begin{equation}
\label{eq:01}
\langle \nabla_{\bx} L(\bx, \btheta), \bx\rangle\leq \tilde{b}-\tilde{m}\|\bx\|^2.
% \textcolor{red}{\langle \nabla_{\bx} U(\bx), \bx\rangle\leq \tilde{b}-\tilde{m}\|\bx\|^2.
%}
\end{equation}
\end{assump}
This assumption ensures samples to move towards the origin regardless the initial point, 
which is standard in proving the geometric ergodicity of dynamical systems, see e.g. \citet{mattingly02, Maxim17, Xu18}.

\begin{assump}[Gradient noise] 
\label{ass4}
The stochastic gradient is unbiased, that is, 
\begin{equation*}
\E[\nabla_{\bx}\widetilde U(\bx_{k})-\nabla_{\bx} U(\bx_{k})]=0;
\end{equation*}
in addition, there exist some constants $M>0$ and 
$B>0$ such that
\begin{equation*} 
\E [ \|\nabla_{\bx}\widetilde U(\bx_{k})-\nabla_{\bx} U(\bx_{k})\|^2 ] \leq M^2 \|\bx\|^2+B^2,
\end{equation*}
where the expectation $\E[\cdot]$ is taken with respect to the distribution of the noise component in $\nabla_{\bx} \widetilde{U}(\bx)$.
\end{assump}






Lemma \ref{convex_appendix__} establishes a stability condition for CSGLD, which implies potential 
convergence of $\btheta_k$.

\begin{lemma}[Stability, restatement of Lemma \ref{convex_main}]
\label{convex_appendix__} 
%Suppose that the batch size $n$ is sufficiently large, the sample space partition is fine, and the learning rate $\epsilon$ is sufficiently sma
Suppose that Assumptions  \ref{ass2a}-\ref{ass4}  hold. 
For any $\btheta \in \bTheta$, $\langle h(\btheta), \btheta - \btheta_{\star}\rangle \leq  -\phi\|\btheta - \btheta_{\star}\|^2+\mathcal{O}\left(\sup_{\bx} \Var(\xi_n(\bx))+\epsilon+\frac{1}{m}\right)$, where $\phi=\inf_{\btheta} Z_{\btheta}^{-1}>0$, $\theta_{\star}=(\int_{\MX_1}\pi(\bx)d\bx,\int_{\MX_2}\pi(\bx)d\bx,\ldots,\int_{\MX_m}\pi(\bx)d\bx)$, $\Var(\xi_n(\cdot))$ denotes the variance of the noise of the stochastic energy estimator $\xi_n(\cdot)$ of batch size $n$ and it 
decays to $0$ as $n\rightarrow N$.
\end{lemma}

\begin{proof}
 Let $\varpi_{\Psi_{\btheta}}(\bx)\propto\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}$ denote a theoretical invariant measure of SGLD, where 
  $\Psi_{\btheta}(u)$ is a fixed
  piecewise continuous function given by 
\begin{equation}\label{new_design_appendix}
\Psi_{\btheta}(u)= \sum_{i=1}^m \left(\theta(i-1)e^{(\log\theta(i)-\log\theta(i-1)) \frac{u-u_{i-1}}{\Delta u}}\right) 1_{u_{i-1} < u \leq u_i},
\end{equation}
 the full data is used 
 in determining the indexes of subregions, and the learning rate converges to zero. 
 %Let  $\varpi_{\btheta}(\bx)$ denote the empirical 
 %measure of SGLD where the mini-batch of data is used 
 %in determining the indexes of subregions. Obviously, 
 %. 
% According to the convergence theory 
 %of SGLD, see e.g., \citep{Sato2014ApproximationAO}, \citep{DalalyanK2017}, \citep{SongLeSGLD2020} and \citep{bhatia2019bayesian},  
%the empirical measure ${\varpi}_{\btheta}(\bx)$
%of CSGLD converges to $\varpi_{\Psi_{\btheta}}(\bx)$ as the mini-batch  size $n$ approaches the full data size $N$ and the learning rate $\epsilon$ converges to zero. 
 In addition, we 
 define a piece-wise constant function 
 \[
 \widetilde{\Psi}_{\btheta}=\sum_{i=1}^m \theta(i) 1_{u_{i-1} < u \leq u_{i}},
 \]
 and a theoretical measure 
 $\varpi_{\widetilde{\Psi}_{\btheta}}(\bx) \propto \frac{\pi(\bx)}{\theta^{\zeta}(J(\bx))}$. 
 Obviously, as the sample space partition becomes 
 fine and fine, i.e., $u_1 \to u_{\min}$, $u_{m-1}\to u_{\max}$ and $m \to \infty$, we have  
 $\|\widetilde{\Psi}_{\btheta}-\Psi_{\btheta}\|\to 0$ and $\| 
 \varpi_{\widetilde{\Psi}_{\btheta}}(\bx)- 
 \varpi_{\Psi_{\btheta}}(\bx) \|\to 0$, where 
 $u_{\min}$ and $u_{\max}$ denote the minimum and maximum of $U(\bx)$, respectively. 
 Without loss of generality, we assume $u_{\max}<\infty$. Otherwise, $u_{\max}$ can be set to a value such that $\pi(\{\bx: U(\bx)>u_{\max}\})$ is sufficiently small. 
 
 

%By adaptively simulating from $\varpi_{\Psi_{\btheta}}(\bx)\propto\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}$, where \begin{equation}
%    \label{psi_define}
%    \Psi_{\btheta}(u)= \sum_{i=1}^m \left(\theta(i-1)e^{(\log\theta(i)-\log\theta(i-1)) \frac{u-u_{i-1}}{\Delta u}}\right) 1_{u_{i-1} < u \leq u_i},
%\end{equation}
%the random field $\widetilde H_i(\btheta,\bx)$ acts on an empirical measure $\varpi_{\btheta}(\bx)$ which asymptotically approximates the invariant measure $\varpi_{\Psi_{\btheta}}(\bx)$ as $\epsilon\rightarrow 0$ and $n\rightarrow N$. Meanwhile, $\varpi_{\btheta}(\bx):= \frac{1}{Z_{\btheta}} 
%\frac{\pi(\bx)}{\theta^{\zeta}(J(\bx))}$, where $Z_{\btheta}=\sum_{i=1}^m \frac{\int_{\bchi_i \pi(\bx)d\bx}}{\theta(i)^{\zeta}}$, is sufficiently close to $\varpi_{\Psi_{\btheta}}(\bx)$ by Lemma \ref{partition_order}. 

For each $i \in \{1,2,\ldots,m\}$, the random field $\widetilde H_i(\btheta,\bx)={\theta}^{\zeta}(J_{\widetilde U}(\bx))\left(1_{i\geq J_{\widetilde U}(\bx)}-{\theta}(i)\right)$ is a biased estimator of $ H_i(\btheta,\bx)={\theta}^{\zeta}( J(\bx))\left(1_{i\geq J(\bx)}-{\theta}(i)\right)$. By Lemma 4 of \citep{icsgld}, the bias caused by the mini-batch energy estimator follows $\E[\widetilde{H}(\btheta,\bx)-H(\btheta,\bx)]=O\left(\sup_{\bx} \Var(\xi_n(\bx))\right)$, where $\xi_n(\cdot)$ is the noisy energy estimator of batch size $n$ and $\Var(\cdot)$ denotes the variance.

First, let's compute the mean-field $h(\btheta)$ with respect to the empirical measure $\varpi_{\btheta}(\bx)$:
\begin{equation}
\small
\label{iiii}
\begin{split} 
        h_i(\btheta)&=\int_{\MX} \widetilde H_i(\btheta,\bx) 
         \varpi_{\btheta}(\bx) d\bx
         =\int_{\MX} H_i(\btheta,\bx) 
         \varpi_{\btheta}(\bx) d\bx+O\left(\sup_{\bx} \Var(\xi_n(\bx))\right)\\
         &=\ \int_{\MX} H_i(\btheta,\bx) \left( \underbrace{\varpi_{\widetilde{\Psi}_\btheta}(\bx)}_{\text{I}_1} \underbrace{-\varpi_{\widetilde{\Psi}_\btheta}(\bx)+\varpi_{\Psi_{\btheta}}(\bx)}_{\text{I}_2: \text{piece-wise approximation}}\underbrace{-\varpi_{\Psi_{\btheta}}(\bx)+\varpi_{\btheta}(\bx)}_{\text{I}_3: \text{discretization}}\right) d\bx+O\left(\sup_{\bx} \Var(\xi_n(\bx))\right).\\
\end{split}
\end{equation}

(i) For the term $\text{I}_1$, we have
\begin{equation}
\begin{split}
\label{i_1}
    \int_{\MX} H_i(\btheta,\bx) 
     \varpi_{\widetilde{\Psi}_\btheta}(\bx) d\bx&=\frac{1}{Z_{\btheta}} \int_{\MX} {\theta}^{\zeta}(J(\bx))\left(1_{i= J(\bx)}-{\theta}(i)\right) \frac{\pi(\bx)}{\theta^{\zeta}(J(\bx))} d\bx\\
    &=Z_{\btheta}^{-1}\left[\sum_{k=1}^m \int_{\MX_k} 
     \pi(\bx) 1_{k=i} d\bx -\theta(i)\sum_{k=1}^m\int_{\MX_k} \pi(\bx)d\bx \right] \\
    &=Z_{\btheta}^{-1} \left[\theta_{\star}(i)-\theta(i)\right],
\end{split}
\end{equation}
where $Z_{\btheta}=\sum_{i=1}^m \frac{\int_{\MX_i} \pi(\bx)d\bx}{\theta(i)^{\zeta}}$ denotes the normalizing constant 
of $\varpi_{\widetilde{\Psi}_\btheta}(\bx)$.

(ii) As to the integral $\text{I}_2$. By Lemma \ref{partition_order} and the boundedness of $H(\btheta,\bx)$, we have 
\begin{equation} \label{biasI2}
\int_{\MX} H_i(\btheta,\bx) (-\varpi_{\widetilde{\Psi}_{\btheta}}(\bx)+\varpi_{\Psi_{\btheta}}(\bx)) d\bx= \mathcal{O}\left(\frac{1}{m}\right).
\end{equation}
(iii) Regarding the term $\text{I}_3$, we have for any fixed $\btheta$,
\begin{equation}\label{iiii_2}
    \int_{\MX} H_i(\btheta,\bx) \left(-\varpi_{\Psi_{\btheta}}(\bx)+\varpi_{\btheta}(\bx)\right) d\bx=\mathcal{O}(\epsilon),
\end{equation}
where  the order of $\mathcal{O}(\epsilon)$ follows from Theorem 6 of \citet{Sato2014ApproximationAO}.


Plugging (\ref{i_1}), (\ref{biasI2}) and  \textcolor{black}{(\ref{iiii_2})} into (\ref{iiii}), we have
\begin{equation}\label{h_i_theta}
     h_i(\btheta)=Z_{\btheta}^{-1} \left[\varepsilon\beta_i(\btheta)+\theta_{\star}(i)-\theta(i)\right],
\end{equation}
where $\varepsilon=\mathcal{O}\left(\sup_{\bx} \Var(\xi_n(\bx))+\epsilon+\frac{1}{m}\right)$ and $\beta_i(\btheta)$ is a bounded term such that $Z_{\btheta}^{-1}\varepsilon\beta_i(\btheta)=\mathcal{O}\left(\sup_{\bx} \Var(\xi_n(\bx))+\epsilon+\frac{1}{m}\right)$.

To solve the ODE system with small disturbances, we consider standard techniques in perturbation theory.
%and write $\theta(i)=\theta^{(0)}(i)+\varepsilon\theta^{(1)}(i)+\varepsilon^2\theta^{(2)}(i)+\cdot\cdot\cdot$. Then, it suffices to solve 
%\begin{equation}
%    \varepsilon \beta_i\biggl(\left(\theta^{(0)}(i)+\varepsilon\theta^{(1)}(i)+\varepsilon^2\theta^{(2)}(i)+\cdots,\cdots\right)\biggr)+\theta_{\star}(i)-\biggl(\theta^{(0)}(i)+\varepsilon\theta^{(1)}(i)+\varepsilon^2\theta^{(2)}(i)+\cdot\cdot\cdot\biggr)=0
%\end{equation}
%According to the fundamental theorem of perturbation theory, we have $\theta^{(0)}(i)=\theta_{\star}(i)$ 
%for any $i$, given small enough learning rates, large enough batch sizes, and fine enough partitions.
%In what follows, we can show $\theta^{(1)}(i)=\beta_i(\btheta_{\star})$ also holds for any $i$. The solution is summarized as follows
According to the fundamental theorem of
perturbation theory \citep{Eric}, we can obtain the solution to 
the mean field equation $h(\btheta)=0$: 
\begin{equation}
    \theta(i)=\theta_{\star}(i)+\varepsilon\beta_i(\btheta_{\star}) +\mathcal{O}(\varepsilon^2), \quad i=1,2,\ldots,m,
\end{equation}
which is a stable point in a small neighbourhood of $\btheta_{\star}$.


Considering the positive definite function $\mathbb{V}(\btheta)=\frac{1}{2}\| \btheta_{\star}-\btheta\|^2$ for the mean-field system $h(\btheta)=Z_{\btheta}^{-1} (\varepsilon\beta_i(\btheta)+\btheta_{\star}-\btheta)=Z_{\btheta}^{-1} (\btheta_{\star}-\btheta)+\mathcal{O}(\varepsilon)$, we have
\begin{equation*}
\begin{split}
    \langle h(\btheta), \mathbb{V}(\btheta)\rangle&=\langle h(\btheta), \btheta - \btheta_{\star}\rangle \\
    &= -Z_{\btheta}^{-1}\|\btheta - \btheta_{\star}\|^2+\mathcal{O}(\varepsilon)\\
    &\leq -\phi\|\btheta - \btheta_{\star}\|^2+\mathcal{O}\left(\sup_{\bx} \Var(\xi_n(\bx))+\epsilon+\frac{1}{m}\right),
\end{split}
\end{equation*}
where $\phi=\inf_{\btheta} Z_{\btheta}^{-1}>0$ by
the compactness assumption \ref{ass2a}. This concludes the proof.
\end{proof}


%  For a function $V: \bX \to [1,\infty)$ and a function $q: \bX \to \mR^{m}$, 
%  define the norm
% \[
%  \|q\|_V=\sup_{\bx\in \bX} \frac{\|q(\bx)\|}{V(\bx)},
%  \]
%  where $m$ denotes the dimension of $\btheta$. 
%  Let $\mathcal{L}_V=\{q: \bX \to \mR^{m}, \sup_{x\in \bX} \|q\|_V <\infty\}$.

 
% The following lemma is a restatement of Lemma 1 in \citep{deng2019}, for which the required conditions are 
% clearly satisfied due to the compactness assumption \ref{ass2a}.
% \begin{lemma}[Uniform $L^2$ bounds]
% \label{lemma:1}
% Suppose Assumptions \ref{ass2a}-\textcolor{black}{\ref{ass4}} holds.  Given a small enough learning rate
%  $\ 0<\epsilon<\operatorname{Re}(\tfrac{\tilde{m}-\sqrt{\tilde{m}^2-3M^2}}{3M^2})\wedge 1$,  then 
% $\sup_{k\geq 1} \E[\|\bm{\xeta}_{k}\|^2] < \infty$.
% \end{lemma}

\textcolor{black}{The following is a restatement of Lemma 3.2 \citep{Maxim17}, which holds for any $\btheta$ in the compact space $\bTheta$. Similar results have been shown in \citet{deng2019}.
\begin{lemma}[Uniform $L^2$ bounds]
\label{lemma:1}
Suppose Assumptions \ref{ass2a}, \ref{ass3} and \ref{ass4} hold.  Given a small enough learning rate, then 
$\sup_{k\geq 1} \E[\|\bm{\xeta}_{k}\|^2] < \infty$.
\end{lemma}}

The ensure the perturbations of the stochastic approximation process decays sufficiently fast, we present the following result on the regularity properties.
\begin{lemma}[Solution of Poisson equation]
\label{lyapunov}
Suppose that Assumptions  \ref{ass2a}-\ref{ass4}  hold. 
There is a solution $\mu_{\btheta}(\cdot)$ on $\MX$ to the Poisson equation 
\begin{equation}
    \label{poisson_eqn}
    \mu_{\btheta}(\bm{x})-\mathrm{\Pi}_{\bm{\theta}}\mu_{\bm{\theta}}(\bm{x})=\widetilde H(\bm{\theta}, \bm{x})-h(\bm{\theta}).
\end{equation}
In addition, for all $\bm{\theta}, \bm{\theta}'\in \bm{\bTheta}$, %and a function  $V(\bx)=1+\|\bx\|^2$, 
there exists a constant $C$ such that
\begin{equation}
\begin{split}
\label{poisson_reg}
\E[\|\mathrm{\Pi}_{\bm{\theta}}\mu_{\btheta}(\bx)\|]&\leq C,\\
\E[\|\mathrm{\Pi}_{\bm{\theta}}\mu_{\bm{\theta}}(\bx)-\mathrm{\Pi}_{\bm{\theta}'}\mu_{\bm{\theta'}}(\bx)\|]&\leq C\|\bm{\theta}-\bm{\theta}'\|.\\
\end{split}
\end{equation}
\end{lemma}
\begin{proof} The proof hinges on verifying drift conditions proposed in Section 6 of \citep{andrieu05} and the details have been given in Lemma 6 of \citet{icsgld}.


% The lemma can be proved based on 
% Theorem 13 of  \citet{VollmerZW2016}, 
% whose conditions can be 
% easily verified for CSGLD given the assumptions A1-A4 and 
% Lemma \ref{lemma:1}. The details are omitted. 
\end{proof}
 

Now we are ready to prove the first main result on the 
convergence of $\btheta_k$.
The technique lemmas are listed 
in Section \ref{Lemmasection}. 


\begin{assump}[Learning rate and step size]
\label{ass1}
The learning rate $\{\epsilon_k\}_{k \in \mathrm{N}}$ is a positive non-increasing sequence of real numbers satisfying the conditions 
\[
\lim_k \epsilon_k=0, \quad \sum_{k=1}^{\infty} \epsilon_k=\infty.
\]
%which includes a constant learning rate as a special case.
The step size $\{\omega_{k}\}_{k\in \mathrm{N}}$ is a positive decreasing sequence of real numbers such that
\begin{equation} \label{a1}
\omega_{k}\rightarrow 0, \ \ \sum_{k=1}^{\infty} \omega_{k}=+\infty,\ \  \lim_{k\rightarrow \infty} \inf 2\phi  \dfrac{\omega_{k}}{\omega_{k+1}}+\dfrac{\omega_{k+1}-\omega_{k}}{\omega^2_{k+1}}>0.
\end{equation}
According to \citet{Albert90}, we can choose $\omega_{k}:=\frac{A}{k^{\alpha}+B}$ for some $\alpha \in (\frac{1}{2}, 1]$ and some suitable constants 
 $A>0$ and $B>0$. 
 \end{assump}
 


\begin{theorem}[$L^2$ convergence rate, restatement of Theorem \ref{thm:1}]
\label{latent_convergence}
Suppose Assumptions $\ref{ass2a}$-$\ref{ass1}$ hold. For a sufficiently
large value of $m$, a sufficiently small learning rate sequence  $\{\epsilon_k\}_{k=1}^{\infty}$,  and a sufficiently small
 step  size sequence $\{\omega_k\}_{k=1}^{\infty}$, 
$\{\btheta_k\}_{k=0}^{\infty}$ converges to
 $\btheta_{\star}$ in $L_2$-norm  such that
\begin{equation*}
    \E\left[\|\bm{\theta}_{k}-\btheta_{\star}\|^2\right]=\mathcal{O}\left( \omega_{k}+
    \sup_{i\geq k_0}\epsilon_i+
\frac{1}{m} +\sup_{\bx} \Var(\xi_n(\bx))\right),
\end{equation*}
where $k_0$ is a sufficiently large constant, $\xi_n$ is the noisy energy estimator of batch size $n$, and $\Var(\cdot)$ denotes the variance.
\end{theorem}
%\paragraph{Proof of Theorem \ref{latent_convergence}} 
\begin{proof}
Consider the iterations 
\begin{equation*}
    \bm{\theta}_{k+1}=\bm{\theta}_{k}+\omega_{k+1} \left(\widetilde H(\bm{\theta}_{k}, \bm{x}_{k+1})+\omega_{k+1} \rho(\btheta_k, \bx_{k+1})\right).
\end{equation*}
Define $\bm{T}_{k}=\bm{\theta}_{k}-\btheta_{\star}$. By subtracting $\btheta_{\star}$ from both sides and taking the square and $L_2$ norm,  we have
\begin{equation*}
\small
\begin{split}
    \|\bT_{k+1}\|^2&=\|\bT_k\|^2 +\omega_{k+1}^2 \|\widetilde H(\btheta_k, \bx_{k+1}) + \omega_{k+1}\rho(\btheta_k, \bx_{k+1})\|^2+2\omega_{k+1}\underbrace{\langle \bT_k,  \widetilde H(\bx_{k+1})+\omega_{k+1}\rho(\btheta_k, \bx_{k+1})\rangle}_{\text{D}}.
\end{split}
\end{equation*}

First, by Lemma \ref{convex_property}, there exists a constant $G=4Q^2(1+Q^2)$ such that
\begin{equation}
\label{first_term}
    \| \widetilde H(\btheta_k, \bx_{k+1}) + \omega_{k+1}\rho(\btheta_k, \bx_{k+1})\|^2 \leq G (1+\|\bT_k\|^2).
\end{equation}


Next, by the Poisson equation (\ref{poisson_eqn}), we have
\begin{equation*}
\begin{split}
   \text{D}&=\langle \bT_k,  \widetilde H(\btheta_k, \bx_{k+1})+\omega_{k+1}\rho(\btheta_k, \bx_{k+1}) \rangle\\
   &=\langle \bT_k,  h(\btheta_k)+\mu_{\btheta_k}(\bm{x}_{k+1})-\mathrm{\Pi}_{\bm{\theta}_k}\mu_{\bm{\theta}_k}(\bm{x}_{k+1})+\omega_{k+1}\rho(\btheta_k, \bx_{k+1}) \rangle\\
   &=\underbrace{\langle \bT_k,  h(\btheta_k)\rangle}_{\text{D}_{1}} +\underbrace{\langle\bT_k, \mu_{\btheta_k}(\bm{x}_{k+1})-\mathrm{\Pi}_{\bm{\theta}_k}\mu_{\bm{\theta}_k}(\bm{x}_{k+1})\rangle}_{\text{D}_{2}}+\underbrace{\langle \bT_k, \omega_{k+1}\rho(\btheta_k, \bx_{k+1})\rangle}_{{\text{D}_{3}}}.
\end{split}
\end{equation*}

For the term $\text{D}_1$, by Lemma \ref{convex_appendix__}, we have
\begin{align*}
\E\left[\langle \bm{T}_{k}, h(\bm{\theta}_{k})\rangle\right] &\leq - \phi\E[\|\bm{T}_{k}\|^2]+\mathcal{O}(\sup_{\bx} \Var(\xi_n(\bx))+\epsilon_k+\frac{1}{m}).
\end{align*}
For convenience, in the following context, we denote $\mathcal{O}(\sup_{\bx} \Var(\xi_n(\bx))+\epsilon_k+\frac{1}{m})$ by $\Delta_k$. 


To deal with the term $\text{D}_2$, we make the following decomposition 
\begin{equation*}
\begin{split}
\text{D}_2 &=\underbrace{\langle \bT_k, \mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})-\mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\bx}_{k})\rangle}_{\text{D}_{21}} \\
&+ \underbrace{\langle \bT_k,\mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{x}_{k})- \mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})\rangle}_{\text{D}_{22}}
+ \underbrace{\langle \bT_k,\mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})- \mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\rangle}_{\text{D}_{23}}.\\
\end{split}
\end{equation*}


(\text{i})  From the Markov property, $\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})-\mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{x}_{k})$ forms a martingale difference sequence 
$$\E\left[\langle \bT_k, \mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})-\mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{x}_{k})\rangle |\mathcal{F}_{k}\right]=0, \eqno{(\text{D}_{21})}$$
where  $\mathcal{F}_k$ is a $\sigma$-filter formed by $\{\btheta_0, \bx_1, \btheta_1, \bx_2, \cdots, \bx_k,\btheta_k\}$.

(\text{ii})  By the regularity of the solution of Poisson equation in (\ref{poisson_reg}) and Lemma \ref{theta_lip}, we have 
\begin{equation}
\label{theta_delta}
\E[\|\mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{x}_{k})- \mathrm{\Pi}_{\bm{\theta}_{k-1}}
 \mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})\|]\leq C \|\btheta_k-\btheta_{k-1}\|\leq 2Q C\omega_k.
\end{equation}
Using Cauchy–Schwarz inequality, (\ref{theta_delta}) and the compactness of $\Theta$ in Assumption \ref{ass2a}, we have
$$\small{\E[\langle\bm{T}_{k},\mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{x}_{k})- \mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})\rangle]\leq \E[\|\bT_k\|]\cdot 2Q C\omega_k\leq 4Q^2 C\omega_{k}\leq 5Q^2 C\omega_{k+1}}   \eqno{(\text{D}_{22})},$$
where the last inequality follows from assumption \ref{ass1} and holds for a large enough $k$.

(\text{iii})  For the last term of $\text{D}_{2}$, 
\begin{equation*}
\begin{split}
\small
&\langle \bm{T}_{k},\mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})- \mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\rangle\\
=&\left(\langle \bm{T}_{k}, \mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k}) \rangle- \langle \bm{T}_{k+1}, \mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\rangle\right)\\
&\ \ \ +\left(\langle \bm{T}_{k+1}, \mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\rangle-\langle \bm{T}_{k}, \mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\rangle\right)\\
=&{({z}_{k}-{z}_{k+1})}+{\langle \bm{T}_{k+1}-\bm{T}_{k}, \mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\rangle},\\
\end{split}
\end{equation*}
where ${z}_{k}=\langle \bm{T}_{k}, \mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})\rangle$. By the regularity assumption (\ref{poisson_reg}) and Lemma \ref{theta_lip}, 
$$\E\langle \bm{T}_{k+1}-\bm{T}_{k}, \mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\rangle\leq   \E[\|\bm{\theta}_{k+1}-\bm{\theta}_{k}\|] \cdot \E[\|\mathrm{\Pi}_{\bm{\theta}_{k}}\mu_{\bm{\theta}_{k}}(\bm{\xeta}_{k+1})\|] \leq 2Q C \omega_{k+1}.\eqno{(\text{D}_{23})}$$


Regarding $\text{D}_3$, since $\rho(\btheta_k, \bx_{k+1})$ is bounded, applying Cauchy–Schwarz inequality gives
$${\E[\langle \bT_k, \omega_{k+1}\rho(\btheta_k, \bx_{k+1}))]\leq 2Q^2\omega_{k+1}} \eqno{(\text{D}_{3})}$$

Finally, adding (\ref{first_term}), $\text{D}_1$, $\text{D}_{21}$, $\text{D}_{22}$, $\text{D}_{23}$ and $\text{D}_3$ together, it follows that for a constant $C_0 = G+10Q^2C+4QC+4Q^2$,
\begin{equation}
\begin{split}
\label{key_eqn}
\E\left[\|\bm{T}_{k+1}\|^2\right]&\leq (1-2\omega_{k+1}\phi+G\omega^2_{k+1} )\E\left[\|\bm{T}_{k}\|^2\right]+C_0\omega^2_{k+1} +2\Delta_k\omega_{k+1} +2\E[z_{k}-z_{k+1}]\omega_{k+1}.
\end{split}
\end{equation}
Moreover, from (\ref{compactness}) and (\ref{poisson_reg}), $\E[|z_{k}|]$ is upper bounded by
\begin{equation}
\begin{split}
\label{condition:z}
\E[|z_{k}|]=\E[\langle \bm{T}_{k}, \mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})\rangle]\leq \E[\|\bT_k\|]\E[\|\mathrm{\Pi}_{\bm{\theta}_{k-1}}\mu_{\bm{\theta}_{k-1}}(\bm{x}_{k})\|]\leq 2QC.
\end{split}
\end{equation}



According to Lemma $\ref{lemma:4}$, we can choose $\lambda_0$ and $k_0$ such that 
\begin{align*}
\E[\|\bm{T}_{k_0}\|^2]\leq \psi_{k_0}=\lambda_0 \omega_{k_0}+\frac{1}{\phi}\sup_{i\geq k_0}\Delta_{i},
\end{align*}
which satisfies the conditions ($\ref{lemma:3-a}$) and ($\ref{lemma:3-b}$) of Lemma $\ref{lemma:3-all}$. Applying Lemma $\ref{lemma:3-all}$ leads to
\begin{equation}
\begin{split}
\label{eqn:9}
\E\left[\|\bm{T}_{k}\|^2\right]\leq \psi_{k}+\E\left[\sum_{j=k_0+1}^{k}\Lambda_j^k \left(z_{j-1}-z_{j}\right)\right],
\end{split}
\end{equation}
where $\psi_{k}=\lambda_0 \omega_{k}+\frac{1}{\phi}\sup_{i\geq k_0}\Delta_{i}$ for all $k>k_0$. Based on ($\ref{condition:z}$) and the increasing condition of $\Lambda_{j}^k$ in Lemma $\ref{lemma:2}$, we have
\begin{equation}
\small
\begin{split}
\label{eqn:10}
&\E\left[\left|\sum_{j=k_0+1}^{k} \Lambda_j^k\left(z_{j-1}-z_{j}\right)\right|\right]
=\E\left[\left|\sum_{j=k_0+1}^{k-1}(\Lambda_{j+1}^k-\Lambda_j^k)z_j-2\omega_{k}z_{k}+\Lambda_{k_0+1}^k z_{k_0}\right|\right]\\
\leq& \sum_{j=k_0+1}^{k-1}2(\Lambda_{j+1}^k-\Lambda_j^k)QC+\E[|2\omega_{k} z_{k}|]+2\Lambda_k^k QC\\
\leq& 2(\Lambda_k^k-\Lambda_{k_0}^k)QC+2\Lambda_k^k QC+2\Lambda_k^k QC\\
\leq& 6\Lambda_k^k QC.
\end{split}
\end{equation}


Given $\psi_{k}=\lambda_0 \omega_{k}+\frac{1}{\phi}\sup_{i\geq k_0}\Delta_{i}$ which satisfies the conditions ($\ref{lemma:3-a}$) and ($\ref{lemma:3-b}$) of Lemma $\ref{lemma:3-all}$,
it follows from (\ref{eqn:9}) and (\ref{eqn:10}) 
that  the following inequality holds for any $k>k_0$,
 
\begin{equation*}
\E[\|\bm{T}_{k}\|^2]\leq \psi_{k}+6\Lambda_k^k QC=\left(\lambda_0+12QC\right)\omega_{k}+\frac{1}{\phi}\sup_{i\geq k_0}\Delta_{i}=\lambda \omega_{k}+\frac{1}{\phi}\sup_{i\geq k_0}\Delta_{i},
\end{equation*}
where $\lambda=\lambda_0+12QC$, $\lambda_0=\frac{2G\sup_{i\geq k_0} \Delta_i + 2C_0\phi}{C_1\phi}$, $\small{C_1=\lim \inf 2\phi \dfrac{\omega_{k}}{\omega_{k+1}}+\dfrac{\omega_{k+1}-\omega_{k}}{\omega^2_{k+1}}>0}$, $C_0=G+5Q^2C+2QC+2Q^2$ and $G=4 Q^2(1+Q^2)$.
\end{proof}

\subsection{Technical lemmas} \label{Lemmasection}

\begin{lemma}\label{partition_order}
Suppose Assumption \ref{ass2a} holds, and $u_1$ and 
$u_{m-1}$ are fixed such that $\Psi(u_1)>\nu$ and $\Psi(u_{m-1})>1-\nu$ for some small constant $\nu>0$. For any bounded function $f(\bx)$, we have 
\label{m_order}
\begin{equation}\label{i_2}
    \int_{\MX} f(\bx)\left(\varpi_{\Psi_{\btheta}}(\bx)-\varpi_{\widetilde\Psi_{\btheta}}(\bx)\right) d\bx=\mathcal{O}\left(\frac{1}{m}\right).
\end{equation}
\end{lemma}

\begin{proof}
Recall that $\varpi_{\widetilde\Psi_{\btheta}}(\bx)= \frac{1}{Z_{\btheta}} 
\frac{\pi(\bx)}{\theta^{\zeta}(J(\bx))}$ and $\varpi_{\Psi_{\btheta}}(\bx)=\frac{1}{Z_{\Psi_{\btheta}}}\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}$. Since $f(\bx)$ is bounded, 
it suffices to show 
\begin{equation}
\begin{split}
    &\int_{\MX} \frac{1}{Z_{\btheta}} 
\frac{\pi(\bx)}{\theta^{\zeta}(J(\bx))}-\frac{1}{Z_{\Psi_{\btheta}}}\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))} d\bx\\
\leq &\int_{\MX} \left|\frac{1}{Z_{\btheta}} 
\frac{\pi(\bx)}{\theta^{\zeta}(J(\bx))}-\frac{1}{Z_{\btheta}}\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}\right|d\bx+\int_{\MX}\left|\frac{1}{Z_{\btheta}}\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}-\frac{1}{Z_{\Psi_{\btheta}}}\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}\right| d\bx\\
=&\underbrace{\frac{1}{Z_{\btheta}}\sum_{i=1}^m \int_{\MX_i} \left| 
\frac{\pi(\bx)}{\theta^{\zeta}(i)}-\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}\right|d\bx}_{\text{I}_1}+\underbrace{\sum_{i=1}^m\left|\frac{1}{Z_{\btheta}}-\frac{1}{Z_{\Psi_{\btheta}}}\right|\int_{\MX_i}\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))} d\bx}_{\text{I}_2}=\mathcal{O}\left(\frac{1}{m}\right),\\
\end{split}
\end{equation}
where $Z_{\btheta}=\sum_{i=1}^m \int_{\mX_i} \frac{\pi(\bx)}{\theta(i)^{\zeta}}d\bx$, $Z_{\Psi_{\btheta}}=\sum_{i=1}^{m}\int_{\mX_i} \frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}d\bx$, and $\Psi_{\btheta}(u)$ is a piecewise continuous function defined in (\ref{new_design_appendix}).
%such that $\theta(i)<\Psi_{\btheta}(u)\leq \theta(i+1)$ for any $u\in [u_1, \infty)$ and some $i\in\{1,2,..., m-1\}$ that satisfies $u_i< U(\bx)\leq u_{i+1}$. 

By Assumption \ref{ass2a}, $\inf_{\Theta} \theta(i)>0$ for any $i$. 
Further, by the mean-value theorem, which implies $|x^{\zeta}-y^{\zeta}|\lesssim |x-y| z^{\zeta}$ for any $\zeta>0, x\leq y$ and $z\in[x, y]\subset [u_1, \infty)$, we have 
\begin{equation*}
\small
\begin{split}
    \text{I}_1&=\frac{1}{Z_{\btheta}}\sum_{i=1}^m \int_{\MX_i} \left| 
\frac{\theta^{\zeta}(i)-\Psi^{\zeta}_{\btheta}(U(\bx))}{\theta^{\zeta}(i)\Psi^{\zeta}_{\btheta}(U(\bx))}\right|\pi(\bx)d\bx\lesssim \frac{1}{Z_{\btheta}}\sum_{i=1}^m \int_{\MX_i} 
\frac{|\Psi_{\btheta}(u_{i-1})-\Psi_{\btheta}(u_i)|}{\theta^{\zeta}(i)}\pi(\bx)d\bx\\
&\leq \max_i |\Psi_{\btheta}(u_{i}-\Delta u)-\Psi_{\btheta}(u_i)|  \frac{1}{Z_{\btheta}}\sum_{i=1}^m \int_{\MX_i} 
\frac{\pi(\bx)}{\theta^{\zeta}(i)}d\bx=\max_i |\Psi_{\btheta}(u_{i}-\Delta u)-\Psi_{\btheta}(u_i)|\lesssim \Delta u=\mathcal{O}\left(\frac{1}{m}\right),
\end{split}
\end{equation*}
where the last inequality follows by Taylor expansion, 
and the last equality follows as $u_1$ and $u_{m-1}$ 
are fixed. Similarly, we have % the same order for $\text{I}_2$.
\begin{equation*}
    \begin{split}
        \text{I}_2= \left|\frac{1}{Z_{\btheta}}-\frac{1}{Z_{\Psi_{\btheta}}}\right|Z_{\Psi_{\btheta}}=\frac{ |Z_{\Psi_{\btheta}}-Z_{\btheta}|}{Z_{\btheta}}\leq \frac{1}{Z_{\btheta}}\sum_{i=1}^m \int_{\MX_i} \left|\frac{\pi(\bx)}{\theta^{\zeta}(i)}-\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta}(U(\bx))}\right|d\bx=\text{I}_1=\mathcal{O}\left(\frac{1}{m}\right).
    \end{split}
\end{equation*}
The proof can then be concluded by combining the orders of $\text{I}_1$ and $\text{I}_2$. 
\end{proof}

\begin{lemma}
\label{convex_property}
Given $\sup\{\omega_k\}_{k=1}^{\infty}\leq 1$, there exists a constant $G=4 Q^2(1+Q^2)$ such that
\begin{equation} \label{bound2}
\| \widetilde H(\bm{\theta}_k, \bm{\xeta}_{k+1})+\omega_{k+1}\rho(\btheta_k, \bx_{k+1})\|^2 \leq G (1+\|\bm{\theta}_k-\btheta_{\star}\|^2). 
\end{equation}
\end{lemma}
\begin{proof}

According to the compactness condition in Assumption \ref{ass2a}, we have
\begin{equation}
\label{mid_1}
\|\widetilde H(\bm{\theta}_k, \bm{\xeta}_{k+1})\|^2\leq Q^2 (1+\|\bm{\theta}_k\|^2) = 
 Q^2 (1+\|\bm{\theta}_k-\btheta_{\star}+\btheta_{\star}\|^2)\leq Q^2 (1+2\|\bm{\theta}_k-\btheta_{\star}\|^2+2Q^2).
\end{equation}

Therefore, using (\ref{mid_1}), we can show that for a constant $G=4Q^2(1+Q^2)$
\begin{equation*}
\small
\begin{split}
    &\ \ \ \| \widetilde H(\bm{\theta}_k, \bm{\xeta}_{k+1})+\omega_{k+1}\rho(\btheta_k, \bx_{k+1})\|^2 \\
    &\leq 2\|\widetilde H(\bm{\theta}_k, \bm{\xeta}_{k+1})\|^2 + 2\omega_{k+1}^2 \|\rho(\btheta_k, \bx_{k+1})\|^2\\
    &\leq 2Q^2 (1+2\|\bm{\theta}_k-\btheta_{\star}\|^2+2Q^2) + 2Q^2\\
    &\leq 2Q^2 (2+2Q^2+(2+2Q^2)\|\bm{\theta}_k-\btheta_{\star}\|^2)\\
    &\leq G (1+\|\bm{\theta}_k-\btheta_{\star}\|^2).
\end{split}
\end{equation*}
\end{proof}


\begin{lemma}
\label{theta_lip}Given $\sup\{\omega_k\}_{k=1}^{\infty}\leq 1$, we have that
\begin{equation}
\label{lip_theta}
    \|\btheta_{k}-\btheta_{k-1}\|\leq 2\omega_{k} Q
\end{equation}
\end{lemma}

\begin{proof}
Following the update $\btheta_k-\btheta_{k-1}=\omega_k \widetilde H(\bm{\theta}_{k-1}, \bm{x}_{k})+\omega_{k}^2 \rho(\btheta_{k-1}, \bx_{k})$, we have that
$$\|\btheta_{k}-\btheta_{k-1}\|= \|\omega_k \widetilde H(\bm{\theta}_{k-1}, \bm{x}_{k})+\omega_{k}^2 \rho(\btheta_{k-1}, \bx_{k})\|\leq \omega_k\| \widetilde H(\bm{\theta}_{k-1},\bm{x}_{k})\|+\omega_{k}^2\| \rho(\btheta_{k-1}, \bx_{k})\|.$$
By the compactness condition in Assumption \ref{ass2a} and $\sup\{\omega_k\}_{k=1}^{\infty}\leq 1$, (\ref{lip_theta}) can be derived.
\end{proof}



\begin{lemma}
\label{lemma:4}
There exist constants $\lambda_0$ and $k_0$ such that $\forall \lambda\geq\lambda_0$ and $\forall k> k_0$, the sequence $\{\psi_{k}\}_{k=1}^{\infty}$, where $\psi_{k}=\lambda\omega_{k}+\frac{1}{\phi} \sup_{i\geq k_0}\Delta_i$, satisfies
\begin{equation}
\begin{split}
\label{key_ieq}
\psi_{k+1}\geq& (1-2\omega_{k+1}\phi+G\omega_{k+1}^2)\psi_{k}+C_0\omega_{k+1}^2  +2\Delta_k\omega_{k+1}.
\end{split}
\end{equation}
\begin{proof}
By replacing $\psi_{k}$ with $\lambda\omega_{k}+\frac{1}{\phi} \sup_{i\geq k_0}\Delta_i$ in ($\ref{key_ieq}$), it suffices to show
\begin{equation*}
\small
\begin{split}
\label{lemma:loss_control}
\lambda \omega_{k+1}+\frac{1}{\phi} \sup_{i\geq k_0}\Delta_i\geq& (1-2\omega_{k+1}\phi+G\omega_{k+1}^2)\left(\lambda \omega_{k}+\frac{1}{\phi} \sup_{i\geq k_0}\Delta_i\right)+C_0\omega_{k+1}^2 + 2\Delta_k\omega_{k+1}.
\end{split}
\end{equation*}

which is equivalent to proving
\begin{equation*}
\small
\begin{split}
&\lambda (\omega_{k+1}-\omega_k+2\omega_k\omega_{k+1}\phi-G\omega_k\omega_{k+1}^2)\geq  \frac{1}{\phi}\sup_{i\geq k_0}\Delta_i(-2\omega_{k+1}\phi+G\omega_{k+1}^2 )+C_0\omega_{k+1}^2+ 2\Delta_k\omega_{k+1}.
\end{split}
\end{equation*}


Given the step size condition in ($\ref{a1}$), we have $$\small{\omega_{k+1}-\omega_{k}+2 \omega_{k}\omega_{k+1}\phi \geq C_1 \omega_{k+1}^2},$$ 
where $\small{C_1=\lim \inf 2\phi  \dfrac{\omega_{k}}{\omega_{k+1}}+\dfrac{\omega_{k+1}-\omega_{k}}{\omega^2_{k+1}}>0}$. Combining $-\sup_{i\geq k_0}\Delta_i\leq \Delta_k$, it suffices to prove
\begin{equation}
\begin{split}
\label{loss_control-2}
\lambda \left(C_1-G\omega_{k}\right)\omega^2_{k+1}\geq  \left(\frac{G}{\phi} \sup_{i\geq k_0}\Delta_i+C_0\right)\omega^2_{k+1}.
\end{split}
\end{equation}


It is clear that for a large enough $k_0$ and $\lambda_0$ such that $\omega_{k_0}\leq \frac{C_1}{2G}$, $\lambda_0=\frac{2G\sup_{i\geq k_0} \Delta_i + 2C_0\phi}{C_1\phi}$, the desired conclusion ($\ref{loss_control-2}$) holds for all such $k\geq k_0$ and $\lambda\geq \lambda_0$.
\end{proof}
\end{lemma}

The following lemma is a restatement of Lemma 25 (page 247) from \citet{Albert90}.
\begin{lemma}
\label{lemma:2}
Suppose $k_0$ is an integer satisfying
$\inf_{k> k_0} \dfrac{\omega_{k+1}-\omega_{k}}{\omega_{k}\omega_{k+1}}+2\phi-G\omega_{k+1}>0$ 
for some constant $G$. 
Then for any $k>k_0$, the sequence $\{\Lambda_k^K\}_{k=k_0, \ldots, K}$ defined below is increasing and uppered bounded by $2\omega_{k}$
\begin{equation}  
\Lambda_k^K=\left\{  
             \begin{array}{lr}  
             2\omega_{k}\prod_{j=k}^{K-1}(1-2\omega_{j+1}\phi+G\omega_{j+1}^2) & \text{if $k<K$},   \\  
              & \\
             2\omega_{k} &  \text{if $k=K$}.
             \end{array}  
\right.  
\end{equation} 
\end{lemma}


\begin{lemma}
\label{lemma:3-all}
Let $\{\psi_{k}\}_{k> k_0}$ be a series that satisfies the following inequality for all $k> k_0$
\begin{equation}
\begin{split}
\label{lemma:3-a}
\psi_{k+1}\geq &\psi_{k}\left(1-2\omega_{k+1}\phi+G\omega^2_{k+1}\right)+C_0\omega^2_{k+1} + 2 \Delta_k\omega_{k+1},
\end{split}
\end{equation}
and assume there exists such $k_0$ that 
\begin{equation}
\begin{split}
\label{lemma:3-b}
\E\left[\|\bm{T}_{k_0}\|^2\right]\leq \psi_{k_0}.
\end{split}
\end{equation}
Then for all $k> k_0$, we have
\begin{equation}
\begin{split}
\label{result}
\E\left[\|\bm{T}_{k}\|^2\right]\leq \psi_{k}+\sum_{j=k_0+1}^{k}\Lambda_j^k (z_{j-1}-z_j).
\end{split}
\end{equation}
\end{lemma}

\begin{proof}
We prove by the induction method. Assuming (\ref{result}) is true and applying (\ref{key_eqn}), we have that 
\begin{equation*}
\small
\begin{split}
    \E\left[\|\bm{T}_{k+1}\|^2\right]&\leq (1-2\omega_{k+1}\phi+\omega^2_{k+1} G)(\psi_{k}+\sum_{j=k_0+1}^{k}\Lambda_j^k (z_{j-1}-z_j))\\
    &\ \ \ \ \ \ \ \ +C_0\omega^2_{k+1} +2 \Delta_k\omega_{k+1}+2\omega_{k+1}\E[z_{k}-z_{k+1}]\\
\end{split}
\end{equation*}

Combining (\ref{key_ieq}) and Lemma.\ref{lemma:2}, respectively, we have
\begin{equation*}
\small
\begin{split}
    \E\left[\|\bm{T}_{k+1}\|^2\right]&\leq  \psi_{k+1}+(1-2\omega_{k+1}\phi+\omega^2_{k+1} G)\sum_{j=k_0+1}^{k}\Lambda_j^k (z_{j-1}-z_j)+2\omega_{k+1}\E[z_{k}-z_{k+1}]\\
    & \leq \psi_{k+1}+\sum_{j=k_0+1}^{k}\Lambda_j^{k+1} (z_{j-1}-z_j)+\Lambda_{k+1}^{k+1}\E[z_{k}-z_{k+1}]\\
    & \leq \psi_{k+1}+\sum_{j=k_0+1}^{k+1}\Lambda_j^{k+1} (z_{j-1}-z_j).\\
\end{split}
\end{equation*}
\end{proof}


\section{Ergodicity and dynamic importance sampler}
% \setcounter{lemma}{0}

\label{ergodicity}
Our interest is to analyze the deviation between the weighted averaging estimator $\frac{1}{k}\sum_{i=1}^k\theta_{i}^{\zeta}( J_{\widetilde U}(\bx_i)) f(\bx_i)$ and posterior expectation $\int_{\MX}f(\bx)\pi(d\bx)$ for a \textcolor{black}{bounded} function $f$. To accomplish this analysis, we first study the convergence of the 
posterior sample mean $\frac{1}{k}\sum_{i=1}^k f(\bx_i)$ 
to the posterior expectation $\bar{f}=\int_{\MX}f(\bx)\varpi_{\Psi_{\btheta_{\star}}}(\bx)(d\bx)$ and then extend it to $\int_{\MX}f(\bx)\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx)$. The key tool for establishing the ergodic theory is still the Poisson equation 
which is used to characterize the fluctuation 
between $f(\bx)$ and $\bar f$: 
\begin{equation}
    \mathcal{L}g(\bx)=f(\bx)-\bar f,
\end{equation}
where $g(\bx)$ is the solution of the Poisson equation, and $\mathcal{L}$ is the infinitesimal generator of the Langevin diffusion 
\begin{equation*}
    \mathcal{L}g:=\langle\nabla g, \nabla L(\cdot, \btheta_{\star})\rangle+\textcolor{black}{\tau}\nabla^2g.
\end{equation*}

To control the perturbations of $\frac{1}{k}\sum_{i=1}^k f(\bx_i)-\bar f$ and enables convergence of the weighted averaging estimate, \citet{Chen15} impose the following regularity conditions on the solution $g(\bx)$:
\paragraph{Regularity} Given a sufficiently smooth function $g(\bx)$ and a function $\mathcal{V}(\bx)$ such that $\|D^k g\|\lesssim \mathcal{V}^{p_k}(\bx)$ for some 
constants $p_k>0$, where $k\in\{0,1,2,3\}$. In addition, $\mathcal{V}^p$ has a bounded expectation, i.e., $\sup_{\bx} \E[\mathcal{V}^p(\bx)]<\infty$; and $\mathcal{V}$ is smooth, i.e. $\sup_{s\in\{0, 1\}} \mathcal{V}^p(s\bx+(1-s)\by)\lesssim \mathcal{V}^p(\bx)+\mathcal{V}^p(\by)$ for all $\bx,\by\in\MX$ and $p\leq 2\max_k\{p_k\}$. 

For stronger but verifiable conditions, we refer readers to \citet{VollmerZW2016}. For further verifications, \citet{Mackey18} showed that the 0th, 1st and 2nd order of the regularity can be verified given standard smoothness and dissipative assumptions. In what follows, we present a lemma, which is majorly adapted from Theorem 2 of \citet{Chen15} with a fixed learning rate $\epsilon$. 

%\begin{assump}[Regularity condition on the target distribution]  \label{ass7} The target distribution $\pi(\bx)$ has finite second moments, i.e., $\int_{\MX} \|\bx\|^2 \pi(\bx) d\bx < \infty$. 
%\end{assump}

\begin{lemma}[Convergence of the Averaging Estimators, restatement of Lemma \ref{avg_converge}]
\label{avg_converge_appendix}
Suppose Assumptions \ref{ass2a}-\ref{ass1} hold.
%and that the full data is used in determining the indexes of subregions.  
For any bounded function $f$, 
\begin{equation*}
\small
\begin{split}
    \left|\E\left[\frac{\sum_{i=1}^k f(\bx_i)}{k}\right]-\int_{\MX}f(\bx)\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx\right|&=
    \mathcal{O}\left(\frac{1}{k\epsilon}+\sqrt{\epsilon}+\sqrt{\frac{\sum_{i=1}^k \omega_i}{k}}+ \frac{1}{\sqrt{m}}+
    \sqrt{\sup_{\bx} \Var(\xi_n(\bx))}\right), \\
\end{split}
\end{equation*}
where $k_0$ is a sufficiently large constant, $\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx) \propto  
\frac{\pi(\bx)}{\theta_{\star}^{\zeta}(J(\bx))}$, and $\frac{\sum_{i=1}^k \omega_i}{k} =o(\frac{1}{\sqrt{k}})$ as implied by Assumption \ref{ass1}. 
%$Z_{\btheta_{\star}}=\sum_{i=1}^m \frac{\int_{\MX_i} \pi(\bx)d\bx}{\theta_{\star}^{\zeta}(i)}$}.
\end{lemma}


\begin{proof}
% In the case that the full data is used in determining the indexes of subregions, the CSGLD
% algorithm can be written as follows:
%can view the adaptive algorithm as a standard sampling algorithm with fixed latent variable $\btheta_{\star}$ as follows
We rewrite the CSGLD algorithm as follows:
\begin{equation*}
\begin{split}
    \bm{x}_{k+1}&=\bx_k- \epsilon_k\nabla_{\bx} \widetilde{L}(\bx_k, \btheta_k)+\mathcal{N}({0, 2\epsilon_k \tau\bm{I}})\\
    &=\bx_k- \epsilon_k\left(\nabla_{\bx} 
    \widehat{L}(\bx_k, \btheta_{\star})+{\Upsilon}(\bx_k, \btheta_k, \btheta_{\star})\right)+\mathcal{N}({0, 2\epsilon_k \tau\bm{I}}),
\end{split}
\end{equation*}
where    
$\nabla_{\bx} \widehat{L}(\bx,\btheta)= \frac{N}{n} \left[1+  \frac{\zeta\tau}{\Delta u}  \left(\textcolor{black}{\log \theta({J}(\bx))-\log\theta(({J}(\bx)-1)\vee 1)} \right) \right]  \nabla_{\bx} \widetilde U(\bx)$,  $\nabla_{\bx} \widetilde{L}(\bx,\btheta)$ is as 
defined in Section \ref{Alg:app},
 and the bias term is given by ${\Upsilon}(\bx_k,\btheta_k,\btheta_{\star})=\nabla_{\bx} \widetilde{L}(\bx_k,\btheta_k)-\nabla_{\bx} \widehat{L}(\bx_k,\btheta_{\star})$.
%and is an 
%unbiased estimator of 
%$\nabla_{\bx} {L}(\bx_k,\btheta_k)-\nabla_{\bx} {L}(\bx_k,\btheta_{\star})$.

%By the boundedness of $\Theta$ and   $\inf_{\Theta}\theta(i)>0$, 
% By Assumption \ref{ass4}, Lemma \ref{lemma:1},
% and Eve's law (i.e., the variance decomposition formula),
% it is easy to derive that  $\E\|\nabla_{\bx} \tilde{U}(\bx)\|^2<\infty$. 
% Then, by the triangle inequality and Jensen's inequality, we have

By Assumption \ref{ass2}, we have $\|\nabla_{\bx} U(\bx)\|=\|\nabla_{\bx} U(\bx)-\nabla_{\bx} U(\bx_{\star})\|\lesssim \|\bx-\bx_{\star}\|\leq \|\bx\|+\|\bx_{\star}\|$ for some optimum. Then the $L^2$ upper bound in Lemma \ref{lemma:1} implies that $\nabla_{\bx} U(\bx)$ has a bounded second moment. Combining Assumption \ref{ass4}, we have $\E\left[\|\nabla_{\bx} \widetilde U(\bx)\|^2\right]<\infty$. Further by Eve’s law (i.e., the
variance decomposition formula), it is easy to derive that $\E \left[\| \nabla_{\bx} \widetilde{U}(\bx) \|\right]<\infty$.
%[The previous one is not that straightforward, so I filled in the gaps.]} 
Then, by the triangle inequality and Jensen's inequality, 
\begin{equation}
\label{latent_bias}
\small
\begin{split}
    \|\E[\Upsilon(\bx_k,\btheta_k,\btheta_{\star})]\|&\leq 
    \E[\|\nabla_{\bx} \widetilde{L}(\bx_k, \btheta_k)-\nabla_{\bx} \widetilde{L}(\bx_k, \btheta_{\star})\|] + \E[\|\nabla_{\bx} \widetilde{L}(\bx_k, \btheta_{\star})-\nabla_{\bx} \widehat{L}(\bx_k, \btheta_{\star})\|] \\
    &\lesssim  \E[\|\btheta_k-\btheta_{\star}\|]+\mathcal{O}(\sup_{\bx} \Var(\xi_n(\bx)))\leq \sqrt{\E[\|\btheta_k-\btheta_{\star}\|^2]}+\mathcal{O}(\sup_{\bx} \Var(\xi_n(\bx)))\\
    &\leq \mathcal{O}\left( \sqrt{\omega_{k}+\epsilon+
\frac{1}{m} +\sup_{\bx} \Var(\xi_n(\bx)))}\right),
\end{split}
\end{equation}
where Assumption \ref{ass2a} and Theorem \ref{latent_convergence} are used to derive the smoothness of $\nabla_{\bx} \tilde{L}(\bx, \btheta)$ with respect to $\btheta$, and  $\sup_{\bx} \Var(\xi_n(\bx))$ is the bias caused by the mini-batch evaluation of $U(\bx)$.

The ergodic average based on biased gradients and a fixed learning rate is a direct result of Theorem 2 of  \citet{Chen15}. By simulating from $\varpi_{\Psi_{\btheta_{\star}}}(\bx)\propto\frac{\pi(\bx)}{\Psi^{\zeta}_{\btheta_{\star}}(U(\bx))}$ and combining (\ref{latent_bias}) and Theorem \ref{latent_convergence}, we have 
\begin{equation*}
\small
\begin{split}
    \left|\E\left[\frac{\sum_{i=1}^k f(\bx_i)}{k}\right]-\int_{\MX}f(\bx) \varpi_{\Psi_{\btheta_{\star}}}(\bx)d\bx\right|&\leq \mathcal{O}\left(\frac{1}{k\epsilon}+\epsilon+\frac{\sum_{i=1}^k \|\E[\Upsilon(\bx_k,\btheta_k,\btheta_{\star})]\|}{k}\right)\\
    &\lesssim \mathcal{O}\left(\frac{1}{k\epsilon}+\epsilon+\frac{\sum_{i=1}^k \sqrt{\omega_i+\epsilon+\frac{1}{m}+\sup_{\bx} \Var(\xi_n(\bx))}}{k}\right) \\
    &\leq \mathcal{O}\left(\frac{1}{k\epsilon}+\sqrt{\epsilon}+\sqrt{\frac{\sum_{i=1}^k \omega_i}{k}}+
    \frac{1}{\sqrt{m}}+\sqrt{\sup_{\bx} \Var(\xi_n(\bx))}\right),
\end{split}
\end{equation*}
where the last inequality follows by repeatedly applying the inequality $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$ and 
the inequality $\sum_{i=1}^k \sqrt{\omega_i}\leq \sqrt{k\sum_{i=1}^k \omega_i}$.

For any a bounded function $f(\bx)$, we have $|\int_{\MX}f(\bx) \varpi_{\Psi_{\btheta_{\star}}}(\bx)d\bx -  \int_{\MX}f(\bx) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx|= \mathcal{O}(\frac{1}{m})$ by Lemma \ref{partition_order}. By the triangle inequality, we have 
\begin{equation*}
\small
\begin{split}
    \left|\E\left[\frac{\sum_{i=1}^k f(\bx_i)}{k}\right]-\int_{\MX}f(\bx) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx\right|\leq  \mathcal{O}\left(\frac{1}{k\epsilon}+\sqrt{\epsilon}+\sqrt{\frac{\sum_{i=1}^k \omega_i}{k}}+ \frac{1}{\sqrt{m}}+
    \sqrt{\sup_{\bx} \Var(\xi_n(\bx))}\right),
\end{split}
\end{equation*}
which concludes the proof. 
\end{proof}


Finally, we are ready to show the convergence of the weighted averaging estimator $\frac{\sum_{i=1}^k\theta_{i}
     ^{\zeta}(J_{\widetilde U}(\bx_i)) f(\bx_i)}{\sum_{i=1}^k\theta_{i}^{\zeta}( 
      J_{\widetilde U}(\bx_i))}$ to the posterior mean $\int_{\MX}f(\bx)\pi(d\bx)$.
\begin{theorem}[Convergence of the Weighted Averaging Estimators, restatement of Theorem \ref{w_avg_converge}] Assume Assumptions \ref{ass2a}-\ref{ass1} hold. For any bounded function $f$, we have that 
\label{w_avg_converge_appendix}
\begin{equation*}
\small
\begin{split}
    \left|\E\left[\frac{\sum_{i=1}^k\theta_{i}
     ^{\zeta}(J_{\widetilde U}(\bx_i)) f(\bx_i)}{\sum_{i=1}^k\theta_{i}^{\zeta}( 
      J_{\widetilde U}(\bx_i))}\right]-\int_{\MX}f(\bx)\pi(d\bx)\right|&= \mathcal{O}\left(\frac{1}{k\epsilon}+\sqrt{\epsilon}+\sqrt{\frac{\sum_{i=1}^k \omega_i}{k}}+\frac{1}{\sqrt{m}}+\sqrt{\sup_{\bx} \Var(\xi_n(\bx))}\right). \\
\end{split}
\end{equation*}
\end{theorem}

\begin{proof}

Applying triangle inequality and $|\E[x]|\leq \E[|x|]$, we have
\begin{equation*}
\footnotesize
    \begin{split}
        &\left|\E\left[\frac{\sum_{i=1}^k\theta_{i}
        ^{\zeta}( J_{\widetilde U}(\bx_i)) f(\bx_i)}{\sum_{i=1}^k\theta_{i}^{\zeta}(
         J_{\widetilde U}(\bx_i))}\right]-\int_{\MX}f(\bx)\pi(d\bx)\right|\\
        \leq &\underbrace{\E\left[\left|\frac{\sum_{i=1}^k\theta_{i}^{\zeta}
         (J_{\widetilde U}(\bx_i))f(\bx_i)}
         {\sum_{i=1}^k\theta_{i}^{\zeta}(J_{\widetilde U}(\bx_i)) }-\frac{\sum_{i=1}^k\theta_{i}^{\zeta}
         ({J}(\bx_i))f(\bx_i)}
         {\sum_{i=1}^k\theta_{i}^{\zeta}({J}(\bx_i)) }\right|\right]}_{\text{I}_1}\\
         &\ \ +\underbrace{\E\left[\left|\frac{\sum_{i=1}^k\theta_{i}^{\zeta}
         ({J}(\bx_i))f(\bx_i)}
         {\sum_{i=1}^k\theta_{i}^{\zeta}({J}(\bx_i)) }-\frac{Z_{\btheta_{\star}}\sum_{i=1}^k\theta_{i}^{\zeta} ({J}(\bx_i)) f(\bx_i)}{k}\right|\right]}_{\text{I}_2}\\
        \ \ + &\underbrace{\E\left[\frac{Z_{\btheta_{\star}}}{k}\sum_{i=1}^k\left|\theta_i^{\zeta} ({J}(\bx_i))-\theta_{\star}^{\zeta}
      ({J}(\bx_i))  \right| \cdot |f(\bx_i)|\right]}_{\text{I}_3} +\underbrace{\left|\E\left[\frac{Z_{\btheta_{\star}}}{k}\sum_{i=1}^k\theta_{\star}^{\zeta}
     ({J}(\bx_i)) f(\bx_i)\right]-\int_{\MX}f(\bx)\pi(d\bx)\right|}_{\text{I}_4}.
    \end{split}
\end{equation*}


For the term $\text{I}_1$, consider the bias $\E[\widetilde H(\btheta, \bx)- H(\btheta, \bx)]=O\left(\sup_{\bx} \Var(\xi_n(\bx))\right)$ as defined in the proof of Lemma 
\ref{convex_appendix__}. By applying mean-value theorem, we have 
\begin{equation}
\footnotesize
\begin{split}
    \text{I}_1&=\E\left[\left|\frac{\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         J_{\widetilde U}(\bx_i))f(\bx_i)\right)\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         {J}(\bx_i))\right)-\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         {J}(\bx_i))f(\bx_i)\right)\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         J_{\widetilde U}(\bx_i))\right)}
         {\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         J_{\widetilde U}(\bx_i))\right)\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         {J}(\bx_i))\right)}\right|\right]\\
         %%%%%
         &\lesssim O\left(\sup_{\bx} \Var(\xi_n(\bx))\right) \E\left[\frac{\left(\sum_{i=1}^k\theta_{i}
     ^{\zeta}({J}(\bx_i)) f(\bx_i) \left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         {J}(\bx_i))\right)\right)}{\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         {J}(\bx_i))\right)\left(\sum_{i=1}^k\theta_{i}^{\zeta}(
         {J}(\bx_i))\right)}\right]
         =O\left(\sup_{\bx} \Var(\xi_n(\bx))\right).
\end{split}
\end{equation}

For the term $\text{I}_2$, 
by the boundedness of $\bTheta$ and $f$ and the assumption  $\inf_{\Theta}\theta^{\zeta}(i)>0$, we have
\begin{equation*}
\small
\begin{split}
    \text{I}_2=&\E\left[\left|\frac{\sum_{i=1}^k\theta_{i}^{\zeta}({J}(\bx_i))  f(\bx_i)}{\sum_{i=1}^k\theta_{i}^{\zeta}
    ({J}(\bx_i))
    }\left(1-\sum_{i=1}^k\frac{\theta_i^{\zeta}
    ({J}(\bx_i))
    }{k}Z_{\btheta_{\star}}\right)\right|\right]\\
    %%%%%%
    \lesssim & \E\left[\left|Z_{\btheta_{\star}}\frac{{\sum_{i=1}^k\theta_{i}^{\zeta}
    ({J}(\bx_i))
    }}{k}-1\right|\right]\\
    =&\E\left[\left|Z_{\btheta_{\star}}\sum_{i=1}^m \frac{\sum_{j=1}^k\left( \theta_j^{\zeta}(i)-\theta_{\star}^{\zeta}(i)+\theta_{\star}^{\zeta}(i)\right)1_{
    {J}(\bx_j)=i}}{k}-1\right|\right]\\
    %%%%%%%%%%%
    \leq & \underbrace{\E\left[Z_{\btheta_{\star}}\sum_{i=1}^m \frac{\sum_{j=1}^k\left| \theta_j^{\zeta}(i)-\theta_{\star}^{\zeta}(i)\right| 1_{{J}(\bx_j)=i}}{k} \right]}_{\text{I}_{21}} + \underbrace{\E\left[\left| Z_{\btheta_{\star}}\sum_{i=1}^m \frac{\theta_{\star}^{\zeta}(i)\sum_{j=1}^k  1_{{J}(\bx_j)=i}}{k}-1\right|
    \right]}_{\text{I}_{22}}.\\
\end{split}
\end{equation*}


For $\text{I}_{21}$, by first applying the inequality $|x^{\zeta}-y^{\zeta}|\leq \zeta |x-y| z^{\zeta-1}$ for any $\zeta>0, x\leq y$ and $z\in[x, y]$ based on the mean-value theorem and then applying the Cauchy–Schwarz inequality, we have 
\begin{equation}\label{ii_21}
    \text{I}_{21}\lesssim \frac{1}{k}\E\left[ \sum_{j=1}^k\sum_{i=1}^m\left| \theta_j^{\zeta}(i)-\theta_{\star}^{\zeta}(i)\right| \right]\lesssim  \frac{1}{k}\E\left[ \sum_{j=1}^k\sum_{i=1}^m\left| \theta_j(i)-\theta_{\star}(i)\right| \right]\lesssim  \frac{1}{k}\sqrt{\sum_{j=1}^k\E\left[\left\| \btheta_j-\btheta_{\star}\right\|^2\right]},
\end{equation}
where the compactness of $\Theta$ has been 
used in deriving the second inequality. 

For $\text{I}_{22}$, considering the following relation $$
    1=\sum_{i=1}^m\int_{\MX_i} \pi(\bx)d\bx=\sum_{i=1}^m\int_{\MX_i} \theta_{\star}^{\zeta}(i) \frac{\pi(\bx)}{\theta_{\star}^{\zeta}(i)}d\bx
    =Z_{\btheta_{\star}}\int_{\MX} \sum_{i=1}^m \theta_{\star}^{\zeta}(i) 1_{{J}(\bx)=i}\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx,$$ then we have
% \begin{equation}
% \begin{split}
%     \text{I}_{22}&=\E\left[\left|Z_{\btheta_{\star}}\sum_{i=1}^m \theta_{\star}^{\zeta}(i)\left(\frac{\sum_{j=1}^k 1_{
%     {J}(\bx_j)=i}}{k}-\int_{\bX}1_{
%     {J}(\bx)=i}\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx\right)\right|\right]\\
%     %%%%%
%     &\lesssim \sum_{i=1}^m\E\left[\left|\frac{\sum_{j=1}^k 1_{ {J}(\bx_j)=i}
%     }{k}-\int_{\bX} 1_{{J}(\bx)=i }\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx\right|\right]\\
%     &= \mathcal{O}\left(\frac{1}{k\epsilon}+\epsilon^{0.5}+\sqrt{\frac{\sum_{i=1}^k \omega_k}{k}}+\frac{1}{m^{0.5}}\right),
% \end{split}
% \end{equation}
\begin{equation}
\begin{split}
    \text{I}_{22}&=\E\left[\left| Z_{\btheta_{\star}}\sum_{i=1}^m \frac{\theta_{\star}^{\zeta}(i)\sum_{j=1}^k  1_{{J}(\bx_j)=i}}{k}-Z_{\btheta_{\star}}
    \int_{\MX} \sum_{i=1}^m \theta_{\star}^{\zeta}(i) 1_{{J}(\bx)=i}\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx\right|\right]\\
    &=Z_{\btheta_{\star}} \E\left[\left| \frac{1}{k}\sum_{j=1}^k \left(\sum_{i=1}^m\theta_{\star}^{\zeta}(i)  1_{{J}(\bx_j)=i}\right)-\int_{\MX} \left(\sum_{i=1}^m \theta_{\star}^{\zeta}(i) 1_{{J}(\bx)=i}\right)\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)d\bx\right|\right]\\
    &= \mathcal{O}\left(\frac{1}{k\epsilon}+\sqrt{\epsilon}+\sqrt{\frac{\sum_{i=1}^k \omega_i}{k}}+\frac{1}{\sqrt{m}}+  \sqrt{\sup_{\bx} \Var(\xi_n(\bx))} \right),
\end{split}
\end{equation}
where the last equality follows  from Lemma \ref{avg_converge_appendix} as the \textcolor{black}{step 
function $\sum_{i=1}^m \theta_{\star}^{\zeta}(i) 1_{{J}(\bx)=i}$} is bounded. 



For $\text{I}_3$, by the boundedness of $f$,  
the mean value theorem and Cauchy-Schwarz inequality, 
we have 
\begin{equation}\label{ii_3}
\small
    \begin{split}
        \text{I}_3&\lesssim \E\left[\frac{1}{k}\sum_{i=1}^k\left|\theta_{i}
        ^{\zeta}({J}(\bx_i)) -\theta_{\star}^{\zeta}(
        {J}(\bx_i))\right|\right]\lesssim  \frac{1}{k}\E\biggl[ \sum_{j=1}^k\sum_{i=1}^m\bigl| \theta_j(i)-\theta_{\star}(i)\bigr| \biggr]\lesssim  \frac{1}{k}\sqrt{\sum_{j=1}^k\E\left[\left\| \btheta_j-\btheta_{\star}\right\|^2\right]}.\\
    \end{split}
\end{equation}


For the last term $\text{I}_4$, we first decompose $\int_{\MX} f(\bx) \pi(d\bx)$ into $m$ disjoint regions to facilitate the analysis
\begin{equation}
\label{split_posterior}
\footnotesize
\begin{split}
      \int_{\MX} f(\bx) \pi(d\bx)&=\int_{\cup_{j=1}^m \MX_j}  f(\bx) \pi(d\bx)=\sum_{j=1}^m\int_{\MX_j}\theta_{\star}^{\zeta}(j)  f(\bx) \frac{\pi(d\bx)}{\theta_{\star}^{\zeta}(j)}\\
      &=Z_{\btheta_{\star}}\int_{\MX} \sum_{j=1}^m \theta_{\star}(j)^{\zeta}f(\bx) 1_{
        {J}(\bx_i)=j 
        }\varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx).\\
\end{split}
\end{equation}

Plugging (\ref{split_posterior}) into the last term $\text{I}_4$, we have
% \begin{equation}. %%%%%%%%% m elements of order 1/m doesn't mean order 1/m
% \label{final_i2}
% \small
%     \begin{split}
%         \text{I}_4&=\left|\E\left[\frac{Z_{\btheta_{\star}}}{k}\sum_{i=1}^k\sum_{j=1}^m\theta_{\star}(j)^{\zeta} f(\bx_i)1_{  {J}(\bx_i)=j
%         }\right]-\int_{\bX}f(\bx)\pi(d\bx)\right|\\
%         %%%%
%         &=Z_{\btheta_{\star}}\left|\sum_{j=1}^m\theta_{\star}^{\zeta}(j)\E\left[\frac{1}{k}\sum_{i=1}^k f(\bx_i)
%         1_{ {J}(\bx_i)=j 
%         }\right]-\sum_{j=1}^m\theta_{\star}^{\zeta}(j)\int_{\bX_j}  f(\bx) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx)\right|\\
%         %%%%%%
%         &\leq Z_{\btheta_{\star}}\sum_{j=1}^m\theta_{\star}^{\zeta}(j)\left|\E\left[\frac{1}{k}\sum_{i=1}^k f(\bx_i)1_{
%         {J}(\bx_i)=j 
%         }\right]-\int_{\bX_j}  f(\bx) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx)\right|\\
%     \end{split}
% \end{equation}
\begin{equation}
\label{final_i2}
\small
    \begin{split}
        \text{I}_4&=\left|\E\left[\frac{Z_{\btheta_{\star}}}{k}\sum_{i=1}^k\sum_{j=1}^m\theta_{\star}(j)^{\zeta} f(\bx_i)1_{  {J}(\bx_i)=j
        }\right]-\int_{\MX}f(\bx)\pi(d\bx)\right|\\
        % &=Z_{\btheta_{\star}}\left|\sum_{j=1}^m\theta_{\star}^{\zeta}(j)\E\left[\frac{1}{k}\sum_{i=1}^k f(\bx_i)
        % 1_{ {J}(\bx_i)=j 
        % }\right]-\sum_{j=1}^m\theta_{\star}^{\zeta}(j)\int_{\bX_j}  f(\bx) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx)\right|\\
        % &= Z_{\btheta_{\star}}\left|\sum_{j=1}^m\theta_{\star}^{\zeta}(j)\left(\E\left[\frac{1}{k}\sum_{i=1}^k f(\bx_i)1_{
        % {J}(\bx_i)=j 
        % }\right]-\int_{\bX_j}  f(\bx) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx)\right)\right|\\
        &= Z_{\btheta_{\star}}\left|\E\left[\frac{1}{k}\sum_{i=1}^k \left(\sum_{j=1}^m\theta_{\star}^{\zeta}(j) f(\bx_i)1_{
        {J}(\bx_i)=j 
        }\right)\right]-\int_{\MX}  \left(\sum_{j=1}^m\theta_{\star}^{\zeta}(j) f(\bx_i)1_{
        {J}(\bx_i)=j 
        }\right) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx)\right|\\
    \end{split}
\end{equation}



Applying the function \textcolor{black}{$\sum_{j=1}^m\theta_{\star}^{\zeta}(j) f(\bx_i)1_{
        {J}(\bx_i)=j 
        }$ }
to Lemma \ref{avg_converge_appendix} yields
\begin{equation}
\label{almost_i2}
\small
\begin{split}
      \left|\E\left[\frac{1}{k}\sum_{i=1}^k f(\bx_i)\right]-\int_{\MX}  f(\bx) \varpi_{\widetilde{\Psi}_{\btheta_{\star}}}(\bx)(d\bx)\right| = \mathcal{O}\left(\frac{1}{k\epsilon}+\sqrt{\epsilon}+\sqrt{\frac{\sum_{i=1}^k \omega_i}{k}}+\frac{1}{\sqrt{m}}+\sqrt{\sup_{\bx} \Var(\xi_n(\bx))} \right).\\
\end{split}
\end{equation}

Plugging (\ref{almost_i2}) into (\ref{final_i2}) and combining $\text{I}_{1}$, $\text{I}_{21}$, $\text{I}_{22}$, $\text{I}_3$ and Theorem \ref{latent_convergence}, we have
\begin{equation*}
\small
\begin{split}
      \left|\E\left[\frac{\sum_{i=1}^k\theta_{i}
     ^{\zeta}(J_{\widetilde U}(\bx_i)) f(\bx_i)}{\sum_{i=1}^k\theta_{i}^{\zeta}( 
      J_{\widetilde U}(\bx_i))}\right]-\int_{\MX}f(\bx)\pi(d\bx)\right| = \mathcal{O}\left(\frac{1}{k\epsilon}+\sqrt{\epsilon}+\sqrt{\frac{\sum_{i=1}^k \omega_i}{k}}+\frac{1}{\sqrt{m}}+\sqrt{\sup_{\bx} \Var(\xi_n(\bx))} \right),\\
\end{split}
\end{equation*}
which concludes the proof of the theorem.
    

\end{proof}


\section{More discussions on the algorithm}
\label{ext}

\subsection{An alternative numerical scheme}
\label{alternative_scheme}
In addition to the numerical scheme used in (6) and (8) in the main body, we can also consider the following numerical scheme 
  \begin{equation*} \label{alternative_SGLDeq6}
  \footnotesize
 \begin{split}
  \small{\bx_{k+1}=\bx_k - \epsilon_{k+1} \frac{N}{n} \left[1+ 
   \zeta\tau\frac{\log {\theta}_{k}\big(J_{\widetilde U}(\bx_k) \wedge m\big) - \log{\theta}_{k}\big(J_{\widetilde U}(\bx_k)\big)}{\Delta u}  \right]  
    \nabla_{\bx} \widetilde U(\bx_k) +\sqrt{2 \tau \epsilon_{k+1}} \bw_{k+1}}.
 \end{split}
  \end{equation*}

Such a scheme leads to a similar theoretical result and a better treatment of $\Psi_{\btheta}(\cdot)$ for the subregions that contains stationary points.


\subsection{Bizarre peaks in the Gaussian mixture distribution}


A bizarre peak always indicates that there is a stationary point of the same energy in somewhere of the sample space, as the sample space is partitioned according to the energy function in CSGLD. For example, we study a mixture distribution with asymmetric modes $\pi(x)=1/6 N(-6,1)+5/6 N(4,1)$. Figure \ref{bizzae} shows a bizarre peak at $x$. Although $x$ is not a local minimum, it has the same energy as ``-6'' which is a local minimum. Note that in CSGLD, $x$ and ``-6'' belongs to the same subregion.

\begin{figure}[ht]
\vspace{-0.05in}
  \centering
  \includegraphics[scale=0.27]{figures/energy_barrier_asymmetric_modes_v4.pdf}
  \caption{Explanation of bizarre peaks.}
  \label{bizzae}
  \vspace{-0.05in}
\end{figure}


\subsection{Simulations of multi-modal distributions}

We run all the algorithms with 200,000 iterations and assume the energy and gradient follow the Gaussian distribution with a variance of 0.1. We include an additional quadratic regularizer $(\|\bx\|^2-7)1_{\|\bx\|^2>7}$ to limit the samples to the center region. We use a constant learning rate 0.001 for SGLD, reSGLD, and CSGLD; We adopt the cyclic cosine learning rates with initial learning rate 0.005 and 20 cycles for cycSGLD. The temperature is fixed at 1 for all the algorithms, excluding the high-temperature process of reSGLD, which employs a temperature of 3.  In particular for CSGLD, we choose the step size $\omega_k=\min\{0.003, 10/(k^{0.8}+100)\}$ for learning the latent vector. We fix 100 partitions and each energy bandwidth is set to $0.25$. We choose $\zeta=0.75$.

\subsection{Extension to the scenarios with high-$\zeta$}
\label{more_scalable_target}

% In some complex experiments (e.g. computer vision) with a high-loss function, the fixed point $\btheta_{\star}$ is close to the vector $(1, 0, ..., 0)$, i.e., the first subregion may dominate the probability mass. As a result, estimating $\theta(i)$'s for the high energy subregions can be quite difficult due to the limitation of floating points. 

In some complex big data experiments, the first subregion may dominate the probability mass and estimating $\theta(i)$'s for the high energy subregions can be quite difficult due to the limitation of floating points. If  a small value of $\zeta$ is used, the gradient multiplier $1+ 
   \zeta\tau\frac{\log {\theta}_{\star}(i) - \log{\theta}_{\star}((i-1)\vee 1)}{\Delta u}$ is close to $1$ for any $i$ and the algorithm will perform similarly to SGLD, except with different weights. When a large value of $\zeta$ is used, the stochastic approximation update in Eq.(\ref{def_tilde_H}) is slow \textcolor{red}{since $\theta^{\zeta}$ is close to 0}. To tackle this issue, one solution is to include a high-order bias item in the stochastic approximation:
\begin{equation} \label{regularizer_cslgd}
{\theta}_{k+1}(i)={\theta}_{k}(i)+\omega_{k+1}\left({\theta}_{k}^{\textcolor{red}{\zeta}}(J_{\widetilde U}(\bx_{k+1})+\omega_{k+1} 1_{i\geq J_{\widetilde U}(\bx_{k+1})}\rho)\right)\left(1_{i= J_{\widetilde U}(\bx_{k+1})}-{\theta}_{k}(i)\right), 
\end{equation} 
for $i=1,2,\ldots,m$, where $\rho$ is a constant. As shown early, our convergence theory allows inclusion of such a high-order bias term.
In simulations, the high-order bias term $\omega_{k+1}^2 1_{i\geq J_{\widetilde U}(\bx_{k+1})}\rho$ penalized more on the higher energy regions, and thus accelerates the convergence % of $\btheta_k$  toward the pattern  $(1,0,0,\ldots,0)$ especially 
in the early period.



In the computer vision examples, we set the momentum coefficient  to 0.9 and the weight decay to $25$. For CSGHMC and saCSGHMC, we set $\omega_k=\frac{10}{k^{0.75}+1000}$ and $\rho=1$ in (\ref{regularizer_cslgd}) for both CIFAR10 and CIFAR100,  and set $\zeta=1\times 10^6$ for CIFAR10 and $3\times 10^6$ for CIFAR100. 

\paragraph{Can we make the algorithm more scalable:} The additional term $\rho$ makes the algorithm less appealing in practice. To tackle that issue and make it more scalable to big datasets, we can adopt a more scalable and elegant stochastic approximation scheme proposed in \citet{icsgld}
\begin{equation*} \label{novel_cslgd}
{\theta}_{k+1}(i)={\theta}_{k}(i)+\omega_{k+1} {\theta}_{k}(J_{\widetilde U}(\bx_{k+1})\left(1_{i= J_{\widetilde U}(\bx_{k+1})}-{\theta}_{k}(i)\right).
\end{equation*}

Compared to Eq.(\ref{regularizer_cslgd}), the dependence of $\rho$ is no longer required. Moreover, since $\theta(i)<1$ for any $i\in\{1,2,\cdots, m\}$, $\theta(i)^{\zeta}\approx 0$ when $\zeta\gg 1$, which makes Eq.(\ref{regularizer_cslgd}) hard to update. By contrast, the new scheme doesn't have this issue. Theoretically, a local stability shows that $\theta_k(i)$ converges to a much smoother estimate $(\int_{\MX_i}\pi(\bx)d\bx)^{\frac{1}{\zeta}}$ instead of the original $\int_{\MX_i}\pi(\bx)d\bx$ for $i\in\{1,2,\cdots, m\}$ and $\zeta>1$. Notably, the new target is proven to be easier to estimate for high-energy regions.



% \subsection{UCI datasets}\label{regularizer_UCI}

% \begin{table}[!htb]
%   \centering
% \caption{Hyperparameter setting for UCI datasets.}
%   \begin{tabular}{c|ccccccc}
%     \toprule
%     Dataset &   Energy &  Concrete &   Yacht & Boston & Wine  \\
%     Hyperparameters ($\tau/\zeta$) &   1/1  & 5/1  & 1/2.5 & 25/25 & 5/10 \\
%     \bottomrule
%   \end{tabular}
%   \label{hyperparameter}
%   %\vspace{-0.2in}
% \end{table}


% \subsection{CIFAR10 and CIFAR100}\label{regularizer}

% For all the algorithms, the momentums were set to 0.9. The weight decay was set to $25$ and data augmentation was employed following \citep{Zhong17}.  For CSGHMC and saCSGHMC, the step size follows $\omega_k=\frac{10}{k^{0.75}+1000}$ and we set $\rho=1$ in (\ref{regularizer_cslgd}) for both datasets. The sample space was partitioned according to the energy function into 200 subregions with the energy bandwidth $\Delta {u}=1000$ for CIFAR 10 and $\Delta u=5000$ for CIFAR100. For the hyperparameter, we set $\zeta$ as $1\times 10^6$ to CIFAR10 and $3\times 10^6$ for CIFAR100 experiments. 

% In the first set of experiments, all the algorithms utilized a fixed learning rate $\epsilon=2e-7$ and a fixed temperature $\tau=0.01$ under the Bayesian setting.

% In the second set of experiments, we employed a decaying schedule on both learning rates and temperatures (if applicable) to obtain simulated annealing effects. For the learning rate, we fix it at $2e-6$ in the first 400 epochs and then decayed it by a factor of 1.01 at each epoch. For the temperature, it starts from 0.01 and then we consistently decayed it by a factor of 1.01 at each epoch.

\subsection{Number of partitions}
A fine partition will lead to a smaller discretization error, but it may increase the risk in stability. In particular, it leads to large bouncy jumps around optima (a large negative learning rate, i.e., $\frac{\log\theta(2)-\log\theta(1)}{\Delta u}\ll 0$ in formula (8) may be caused there). Empirically, we suggest to partition the sample space into a moderate number of subregions, e.g. 10-1000, to balance between stability and discretization error.




 
 
 
 
 



